A note on discrete fractional integral operators on the Heisenberg group

We consider the discrete analogue of a fractional integral operator on the Heisenberg group, for which we are able to prove nearly sharp results by means of a simple argument of a combinatorial nature.

==> format.tex <==



%this puts 1.2 or 1.1 times the normal spacing between lines; this is a nice balance between single and double spacing
%\renewcommand{\baselinestretch}{1.1}


%\setlength{\oddsidemargin}{.5in}   %{.4375in}
%\setlength{\evensidemargin}{.5in} %{.4375in}
%\setlength{\topmargin}{-.5in}  %{-.5625in}
%\setlength{\textheight}{9in}
%\setlength{\textwidth}{6in}

%ORIGINAL SETTINGS WORK FINE; pretty but wastes space
%\setlength{\topmargin}{0in}
%\setlength{\oddsidemargin}{0.5in}
%\setlength{\evensidemargin}{0in}
%\setlength{\textheight}{8.2in}
%\setlength{\textwidth}{5.2in}

%%This setting is for double sided printing and has 1" margins on three sides, 1.5" inch margins on binding side
%\setlength{\topmargin}{-.2in}
%\setlength{\oddsidemargin}{0.5in}
%\setlength{\evensidemargin}{0in}
%\setlength{\textheight}{8.7in}
%\setlength{\textwidth}{6in}

%This setting is for double sided printing and is slightly more generous: 1.2" margins on three sides, 1.6" inch margins on binding side
%\setlength{\topmargin}{0in}
%\setlength{\oddsidemargin}{0.7in}
%\setlength{\evensidemargin}{0.2in}
%\setlength{\textheight}{8.3in}
%\setlength{\textwidth}{5.6in}



%%SETTING UP HEADERS AND FOOTERS
%\pagestyle{fancy} 
%% with this we ensure that the chapter and section
% % headings are in lowercase. 
%%\renewcommand{\chaptermark}[1]{\markright{\thechapter\#1}} 
%\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}} 
%\fancyhf{} % delete current setting for header and footer 
%\fancyhead[LE,RO]{\thepage} 
%\fancyhead[LO]{\leftmark} 
%\fancyhead[RE]{\leftmark} 
%\renewcommand{\headrulewidth}{.5pt} 
%\renewcommand{\footrulewidth}{0pt} 
%\addtolength{\headheight}{14pt} % make space for the rule 

%\fancypagestyle{plain}{% 
%\fancyhead{} % get rid of headers on plain pages 
%\renewcommand{\headrulewidth}{0pt} % and get rid of the line 
%} 
%\headsep=10pt

%This makes it so that even subsubsections are numbered:
\setcounter{secnumdepth}{4}



%%THESIS COMMENTS
%%toggle on to remove thesis comments
%	%\newcommand{\thesis}[1]{}
%%toggle on to show thesis comments
%	\newcommand{\thesis}{}
%%EXTRA THESIS COMMENTS
%%toggle on to remove extra thesis comments
%	\newcommand{\xtra}[1]{}
%%toggle on to show extra thesis comments
%%THESE ARE THE EXTRA FOOTNOTES
%%	\newcommand{\xtra}[1]{\footnote{{\emph{#1}}}}
%%QUESTIONS
%%toggle on to remove question comments
%	\newcommand{\ques}[1]{}
%%toggle on to show question comments
%%	\newcommand{\ques}[1]{{\bfseries \emph{#1}}}

 
\newtheorem{thm}{Theorem}
%\newtheorem*{thm*}{Theorem}
%\newtheorem{prop}{Proposition}
%\newtheorem*{prop*}{Proposition}
%%This makes it so that Lemmas are numbered in the same sequence as propositions
%%\newtheorem{lemma}[prop]{Lemma}
%\newtheorem*{lemma*}{Lemma}
%\newtheorem{cor}{Corollary}[thm]
%\newtheorem*{cor*}{Corollary}
%\newtheorem*{conjecture*}{Conjecture}
%\newtheorem{conjecture}{Conjecture}
%\newtheorem*{com}{Comment}
%\newtheorem*{question}{Question}

%This makes theorems that are lettered rather than numbered
%Courtesy of Phillip Matchett Wood
\newtheorem{letterthm}{Theorem}
\renewcommand{\theletterthm}{\Alph{letterthm}}

\newtheorem{letterlemma}{Lemma}
\renewcommand{\theletterlemma}{\Alph{letterlemma}}


\theoremstyle{definition}
\newtheorem{dfn}{Definition}

%this makes the enumerate option give Roman numerals, not arabic
\renewcommand{\labelenumi}{(\roman{enumi})}


\newcommand{\Leg}[2]{ \left( \frac{#1}{#2} \right)}
\newcommand{\con}{\equiv}
\newcommand{\ncon}{\not\equiv}
\newcommand{\ndiv}{\nmid}
\newcommand{\modd}[1]{\; ( \text{mod} \; #1)}
\newcommand{\bstack}[2]{\substack{#1 \\ #2}}
\newcommand{\tstack}[3]{#1\atop {#2 \atop #3}}
\newcommand{\sprod}[2]{\langle #1, #2 \rangle}
\newcommand{\inv}[1]{\overline{#1}}
\newcommand{\conj}[1]{\overline{#1}}
\newcommand{\maps}{\rightarrow}
\newcommand{\lequiv }{\Longleftrightarrow}
\newcommand{\intersect}{\cap}
\newcommand{\Intersect}{\bigcap}
\newcommand{\bigunion}{\bigcup}
\newcommand{\Union}{\bigcup}
\newcommand{\union}{\cup}
\newcommand{\grad}{\nabla}
\newcommand{\diag}{\text{diag}}
\newcommand{\uhat}[1]{\check{#1}}
\newcommand{\tensor}{\otimes}
\newcommand{\isom}{\cong}
\newcommand{\deriv}[1]{\frac{\partial}{\partial #1}}
\newcommand{\pderiv}[2]{\frac{\partial ^#1}{\partial #2}}
\newcommand{\comp}{\circ}

\newcommand{\Frac}{\text{Frac}}
\newcommand{\Ker}{\text{Ker}}
\newcommand{\poly}{\text{poly}}
\newcommand{\Poly}{\text{Poly}}
\newcommand{\Id}{\text{Id}}
%\newcommand{\gcd}{\text{gcd}}
\newcommand{\lcm}{\text{lcm}}


\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\gam}{\gamma}
\newcommand{\ga}{\gamma}
\newcommand{\del}{\delta}
\newcommand{\ep}{\epsilon}
\newcommand{\ka}{\kappa}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\Sig}{\Sigma}
\newcommand{\sig}{\sigma}
\newcommand{\lam}{\lambda}
\newcommand{\Lam}{\Lambda}
\newcommand{\Ga}{\Gamma}

\newcommand{\uchi}{\underline{\chi}}
\newcommand{\tchi}{\tilde{\chi}}

\newcommand{\A}{\mathcal{A}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Ut}{\scriptscriptstyle{\mathcal{U}}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\V}{\mathcal{V}}

\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Proj}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}


\newcommand{\p}{\mathfrak{p}}
\newcommand{\Nf}{\mathfrak{N}}
\newcommand{\M}{\mathfrak{M}}
\newcommand{\m}{\mathfrak{m}}

\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}

\newcommand{\res}{\text{res}}
\newcommand{\Tr}{\text{Tr}}
\newcommand{\rank}{\text{rank}\,}
\newcommand{\cond}{\text{cond}\,}
\newcommand{\Disc}{\text{Disc}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
